WebGraph: Capturing Advertising and Tracking Information Flows for Robust Blocking

Millions of web users directly depend on ad and tracker blocking tools to protect their privacy. However, existing ad and tracker blockers fall short because of their reliance on trivially susceptible advertising and tracking content. In this paper, we first demonstrate that the state-of-the-art machine learning based ad and tracker blockers, such as AdGraph, are susceptible to adversarial evasions deployed in real-world. Second, we introduce WebGraph, the first graph-based machine learning blocker that detects ads and trackers based on their action rather than their content. By building features around the actions that are fundamental to advertising and tracking - storing an identifier in the browser, or sharing an identifier with another tracker - WebGraph performs nearly as well as prior approaches, but is significantly more robust to adversarial evasions. In particular, we show that WebGraph achieves comparable accuracy to AdGraph, while significantly decreasing the success rate of an adversary from near-perfect under AdGraph to around 8% under WebGraph. Finally, we show that WebGraph remains robust to a more sophisticated adversary that uses evasion techniques beyond those currently deployed on the web.

==> Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: paper

clean:
	@if [[ -f main.pdf ]]; then \
		rm main.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;

paper:
	latexmk -bibtex -pdf main
	pdflatex -bibtex -interaction=nonstopmode main

==> parts/dataflow.tex <==
%!TEX root = ../main.tex

In this section, we perform the first comparison of \name. We compare it to AdGraph, that contains content and structure features. \St{Now this becomes a short section.}

Research question: Do behavioral features, that go beyond the content and structure of a graph, result in better tracker classification? 

\subsection{Performance evaluation}

In this sub-section, we compare classifiers trained on AdGraph and \name features. Evaluation will be the overall metrics (Precision/Recall/F-score). We do an initial feature importance analysis and notice that the features are dominated by the content related features. This leads to the question of how robust these content features are, and works as a segue to the next section. 


